Generalized scale functions of standard processes with no positive jumps

As a generalization of scale functions of spectrally negative L\'evy processes, we define scale functions of general standard processes with no positive jumps. For this purpose, we utilize excursion measures. Using our new scale functions we study Laplace transforms of hitting times, potential measures and duality.

==> style-j.tex <==
%%%%%%    theorems      %%%%%%
\theoremstyle{definition}
\newtheorem{Thm}{'藝}[section]
\newtheorem{Thma}{'藝}
\renewcommand{\theThma}{\Alph{Thma}}
\newtheorem{Thmb}{'藝}
\renewcommand{\theThmb}{\arabic{section}.\Alph{Thmb}}
\newtheorem{Lem}[Thm]{•â'è}
\newtheorem{Prop}[Thm]{–½'è}
\newtheorem{Cor}[Thm]{Œn}
\newtheorem{Ass}[Thm]{‰¼'è}
\newtheorem{Conj}[Thm]{—\'z}
\newtheorem{Def}[Thm]{'è‹`}
\newtheorem{Rem}[Thm]{'}
\newtheorem{Ex}[Thm]{—á}
\newtheorem{Prob}{–â}[section]
\newcounter{Exami}
\newcommand{\Exam}{\noindent \refstepcounter{Exami} $ \boxed{\arabic{Exami}} $ \ }

\newcommand{\Proof}[2][Ø–¾]{
\begin{proof}[{\bf #1}]
#2
\end{proof}
}
\newcommand{\Solution}[2][‰ð]{
\begin{proof}[{\bf #1}]
#2
\end{proof}
}







